Hardness of Approximating Quantum Code Distance Beyond $\sqrt{N}$

We study the computational complexity of approximating the minimum distance of a stabilizer code. Classically, the minimum distance problem is NP-hard to approximate even to within an additive gap linear in the block length. For quantum codes, however, the reductions of Kapshikar and Kundu and of Grigorescu, Jha and Samperton reach only an additive $O(\sqrt{N})$ gap in the block length $N$. We close this gap and, in a separate direction, initiate the fine-grained study of the problem. We show that no randomized algorithm approximates the distance to within an additive $\alpha N$, for a constant $\alpha > 0$, unless $\mathsf{NP} \subseteq \mathsf{coRP}$. In the fine-grained setting, for every $\varepsilon > 0$, no randomized $2^{(1-\varepsilon)\kappa}\,\mathrm{poly}(N)$-time algorithm computes the distance of a code with $\kappa$ logical qubits unless SETH falls; and no randomized $2^{o(N)}$-time algorithm approximates the distance to within a linear additive gap, on instances where block length, number of logical qubits, and gap are simultaneously linear, unless non-uniform Gap-ETH falls.

==> bibliography.tex <==
\begin{thebibliography}{99}

\bibitem{NC10} M.~A. Nielsen and I.~L. Chuang.
\emph{Quantum Computation and Quantum Information}.
Cambridge University Press, 10th anniversary edition, 2010.

\bibitem{Got97} D.~Gottesman.
\emph{Stabilizer Codes and Quantum Error Correction}.
PhD thesis, Caltech, 1997. arXiv:quant-ph/9705052.

\bibitem{CRSS98} A.~R. Calderbank, E.~M. Rains, P.~W. Shor, N.~J.~A. Sloane.
Quantum error correction via codes over GF(4).
\emph{IEEE Trans.\ Inf.\ Theory}, 44(4):1369--1387, 1998.

\bibitem{KL97} E.~Knill and R.~Laflamme.
Theory of quantum error-correcting codes.
\emph{Phys.\ Rev.\ A}, 55:900--911, 1997.

\bibitem{HEB04} M.~Hein, J.~Eisert, H.~J. Briegel.
Multiparty entanglement in graph states.
\emph{Phys.\ Rev.\ A}, 69:062311, 2004.

\bibitem{HDERVB06} M.~Hein, W.~D\"ur, J.~Eisert, R.~Raussendorf,
M.~Van~den~Nest, H.~J. Briegel.
Entanglement in graph states and its applications.
arXiv:quant-ph/0602096, 2006.

\bibitem{CSSZ09} A.~Cross, G.~Smith, J.~A. Smolin, B.~Zeng.
Codeword stabilized quantum codes.
\emph{IEEE Trans.\ Inf.\ Theory}, 55(1):433--438, 2009.

\bibitem{KK23} U.~Kapshikar, S.~Kundu.
On the hardness of the minimum distance problem of quantum codes.
\emph{IEEE Trans.\ Inf.\ Theory}, 69(10):6293--6302, 2023.


\bibitem{GJS25} E.~Grigorescu, V.~Jha, E.~Samperton.
On the hardness of approximating minimum distances of quantum codes.
In \emph{45th IARCS Annual Conference on Foundations of Software
Technology and Theoretical Computer Science (FSTTCS 2025)}, LIPIcs
vol.~360, Schloss Dagstuhl -- Leibniz-Zentrum f\"ur Informatik, 2025.
arXiv:2509.21469.

 \bibitem{SV19} N.~Stephens-Davidowitz, V.~Vaikuntanathan. SETH-hardness of
   coding problems. In FOCS 2019, pp. 287--301. Full version: ECCC TR19-159.
 \bibitem{IP99} R.~Impagliazzo, R.~Paturi. Complexity of k-SAT. In CCC 1999.
 \bibitem{IPZ01} R.~Impagliazzo, R.~Paturi, F.~Zane. Which problems have
   strongly exponential complexity? JCSS 63(4):512--530, 2001.
 \bibitem{Din16} I.~Dinur. Mildly exponential reduction from gap 3SAT to
   polynomial-gap label-cover. ECCC TR16-128, 2016.
 \bibitem{MR17} P.~Manurangsi, P.~Raghavendra. A birthday repetition theorem
   and complexity of approximating dense CSPs. In ICALP 2017.
 \bibitem{ABV01} A.~Ashikhmin, A.~Barg, S.~Vl\u{a}du\c{t}. Linear codes with
   exponentially many light vectors. J. Combin. Theory Ser. A, 96(2), 2001.


\bibitem{MV05}
P.~B. Miltersen and N.~V. Vinodchandran.
\newblock Derandomizing {A}rthur-{M}erlin games using hitting sets.
\newblock {\em Computational Complexity}, 14(3):256--279, 2005.

\bibitem{BTL10} S.~Bravyi, B.~M.~Terhal, B.~Leemhuis.
Majorana fermion codes.
\emph{New Journal of Physics}, 12:083039, 2010.

\bibitem{SU05}
R.~Shaltiel and C.~Umans.
\newblock Simple extractors for all min-entropies and a new pseudorandom
  generator.
\newblock {\em Journal of the ACM}, 52(2):172--216, 2005.

\bibitem{KvM02}
A.~Klivans and D.~van Melkebeek.
\newblock Graph nonisomorphism has subexponential size proofs unless the
  polynomial-time hierarchy collapses.
\newblock {\em SIAM Journal on Computing}, 31(5):1501--1526, 2002.


\bibitem{DMS03} I.~Dumer, D.~Micciancio, M.~Sudan.
Hardness of approximating the minimum distance of a linear code.
\emph{IEEE Transactions on Information Theory}, 49(1):22--37, 2003.

\bibitem{BGLR25} V.~Bhattiprolu, V.~Guruswami, E.~Lee, X.~Ren.
Inapproximability of finding sparse vectors in codes, subspaces, and
lattices. In FOCS 2025. arXiv:2410.02636.

\bibitem{ESY84} S.~Even, A.~L.~Selman, Y.~Yacobi.
\emph{The complexity of promise problems with applications to
public-key cryptography.} Information and Control, 61(2):159--173,
1984.

\bibitem{Gol06} O.~Goldreich.
\emph{On promise problems: a survey.} In \emph{Theoretical Computer
Science: Essays in Memory of Shimon Even}, LNCS 3895, pp.~254--290,
Springer, 2006.

\end{thebibliography}


